LISA: Increasing Internal Connectivity in DRAM for Fast Data Movement and Low Latency

This paper summarizes the idea of Low-Cost Interlinked Subarrays (LISA), which was published in HPCA 2016, and examines the work's significance and future potential. Contemporary systems perform bulk data movement movement inefficiently, by transferring data from DRAM to the processor, and then back to DRAM, across a narrow off-chip channel. The use of this narrow channel results in high latency and energy consumption. Prior work proposes to avoid these high costs by exploiting the existing wide internal DRAM bandwidth for bulk data movement, but the limited connectivity of wires within DRAM allows fast data movement within only a single DRAM subarray. Each subarray is only a few megabytes in size, greatly restricting the range over which fast bulk data movement can happen within DRAM. Our HPCA 2016 paper proposes a new DRAM substrate, Low-Cost Inter-Linked Subarrays (LISA), whose goal is to enable fast and efficient data movement across a large range of memory at low cost. LISA adds low-cost connections between adjacent subarrays. By using these connections to interconnect the existing internal wires (bitlines) of adjacent subarrays, LISA enables wide-bandwidth data transfer across multiple subarrays with little (only 0.8%) DRAM area overhead. As a DRAM substrate, LISA is versatile, enabling a variety of new applications. We describe and evaluate three such applications in detail: (1) fast inter-subarray bulk data copy, (2) in-DRAM caching using a DRAM architecture whose rows have heterogeneous access latencies, and (3) accelerated bitline precharging by linking multiple precharge units together. Our extensive evaluations show that each of LISA's three applications significantly improves performance and memory energy efficiency on a variety of workloads and system configurations.

==> plots/1c_copy_results.tex <==
\begin{figure}[t]
    \centering
    \subfloat[IPC]{
        \label{fig:1c_ipc}
        \includegraphics[width=\linewidth,height=0.96in, trim=0 8pt 0 0, clip]{plots/gnuplots/1c_copy_ipc.pdf}
        %\includegraphics[scale=1]{plots/gnuplots/1c_copy_ipc.pdf}
    }

    \vspace{-0.17in}
    \subfloat[Energy]{
        \label{fig:1c_e}
        \includegraphics[width=\linewidth,height=0.97in, trim=0 8pt 0 0, clip]{plots/gnuplots/1c_copy_e_v2.pdf}
    }

    \vspace{-0.07in}
    \subfloat[LISA's performance improvement over \baseline as LLC size varies]{
        \label{fig:1c_cache_sweep}
        \includegraphics[width=\linewidth,height=0.93in, trim=0 6pt 0 0, clip]{plots/gnuplots/1c_copy_cache.pdf}
    }

    \caption{Comparison of copy mechanisms in a single-core system. Value (\%)
    on top indicates the improvement of \lisarc-1 over \baselinenorm.}

\label{fig:1c_perf}
\end{figure}


==> plots/4c_copy_results.tex <==
\begin{figure}[h]
    \centering
    \subfloat[Weighted speedup normalized to \baseline]{
        \label{fig:lisa_4c_ws}
        %\includegraphics[width=\linewidth]{plots/gnuplots/4c_copy_ws.pdf}
        \includegraphics[width=\linewidth,height=0.95in]{plots/gnuplots/4c_copy_ws_errbar.pdf}
    }

    \vspace{-0.1in}
    \subfloat[Memory energy efficiency normalized to \baseline]{
        \label{fig:lisa_4c_energy}
        %\includegraphics[width=\linewidth]{plots/gnuplots/4c_copy_e.pdf}
        \includegraphics[width=\linewidth,height=0.95in]{plots/gnuplots/4c_copy_e_errbar.pdf}
    }
    \caption{Four-core system evaluation: (a) weighted speedup and (b)
    memory energy per instruction.}
    \label{fig:4c_copy_perf}
\end{figure}


==> plots/dram_fig.tex <==
\begin{figure*}[t]
    \centering
    \subfloat[DRAM bank organization.]{
        \begin{minipage}{\linewidth/2}
        \begin{center}
        \label{fig:bank}
        \includegraphics[scale=0.90]{plots/bank_org}
        \end{center}
        \end{minipage}
    }
    \subfloat[Open bitline subarray architecture.]{
        \begin{minipage}{\linewidth/2}
        \begin{center}
        \label{fig:subarray}
        \includegraphics[scale=0.90]{plots/open_bitline_sa}
        \end{center}
        \end{minipage}
    }
    \caption{DRAM bank and subarray organization.}
    \label{fig:dram_background}
\end{figure*}


==> plots/villa_compare.tex <==
\begin{figure}[h]
    \centering
    \subfloat[CHARM~\cite{son-isca2013}]{
        %\begin{minipage}{\linewidth/2-0.1in}
        %\begin{center}
        \label{fig:charm}
        \includegraphics[scale=0.9]{plots/charm}
        %\end{center}
        %\end{minipage}
    }
    \hfill
    %\hspace{0.3in}
    \subfloat[TL-DRAM~\cite{lee-hpca2013}]{
        %\begin{minipage}{\linewidth/2-0.1in}
        %\begin{center}
        \label{fig:tldram}
        \includegraphics[scale=.9]{plots/tldram}
        %\end{center}
        %\end{minipage}
    }
    \caption{Drawbacks of existing heterogeneous DRAMs.}
    \label{fig:villa_compare}
\end{figure}


==> sec/tables/4c_copy_norm_ws.tex <==
\begin{table}[h]
\small
\centering
    \setlength{\tabcolsep}{.33em}
    \begin{tabular}{lcc}
      \toprule
      %\textbf{Copy Methods} & Baseline & RC Inter-SA & RC Inter-Bank & RC Intra-SA & LISA-Clone-15\\
      %\midrule
      %\textbf{Weighted Speedup (WS)} & 1.0 & 0.99 & 0.98 & 0.95 \\
      %\textbf{WS Improvement (\%)} & 1.0 & 0.99 & 0.98 & 0.95 \\

      \textbf{Copy Methods} & \textbf{WS} & \textbf{Normalized WS} \\
      \midrule
      Baseline & 1.96 & 1.00\\
      RC Inter-SA & 1.96 & 1.00\\
      RC Inter-Bank & 2.66 & 1.36 \\
      RC Intra-SA & 4.42 & 2.26 \\
      LISA-Clone-15 & 4.17 & 2.13 \\
      LISA-Clone-1 & 4.50 & 2.19 \\
      Ideal & 4.51 & 2.50 \\
      \bottomrule
    \end{tabular}
\caption{Performance comparisons on a 4-core system.}
\label{tab:4c_copy_norm_ws}
\end{table}


==> sec/tables/4c_lisa_sweep.tex <==
\begin{table}[h]
%\small
\fontsize{8.5}{10.2}\selectfont
\centering
    \setlength{\tabcolsep}{.33em}
    \renewcommand{\arraystretch}{1}
    \begin{tabular}{lrrrrrr}
      \toprule
      %\textbf{Copy Distance} & 2 & 4 & 8 & 16 & 32 & 64 \\
      \textbf{Copy Distance} (hops) & 1 & 3 & 7 & 15 & 31 & 63 \\
      \midrule
      \textbf{RISC Copy Latency} (ns) & 148.5 & 164.5 & 196.5 &
          260.5 & 388.5 & 644.5 \\
      %\midrule
      \textbf{WS Improvement} (\%) & 66.2 & 65.3 & 63.3 & 59.6 & 53.0 & 42.4 \\
      %\midrule
      \textbf{DRAM Energy Savings} (\%) & 55.4 & 55.2 & 54.6 & 53.6 & 51.9 & 48.9 \\
      \bottomrule
    \end{tabular}
\caption{Effect of copy distance on \lisarc.}
\label{tab:4c_lisa_sweep}
\vspace{-2pt}
\end{table}


==> sec/tables/copy_tradeoff.tex <==
\begin{table}[h]
\begin{footnotesize}
  \centering
    \begin{tabular}{llll}
        \toprule
        \textbf{Methods} & \textbf{Latency} & \textbf{Copy Range} & \textbf{Copy
    Granularity} \\
        \cmidrule(rl){1-4}

        Baseline & High & All channels & Cache line (64B) \\

        \rcirsa & Medium $\leftrightarrow$ High & All banks & Cache line \\

        \textbf{\lisarc} & Low $\leftrightarrow$ Medium & One bank & Cache line $\leftrightarrow$  Row \\

        \rciasa & Low & One subarray & Row (8KB) \\

        \bottomrule
    \end{tabular}
    %\begin{tabular}{lllll}
    %    \toprule
    %    Methods & Latency & Copy Range & Copy Granularity & Energy\\
    %    \cmidrule(rl){1-5}

    %    Baseline & High & All channels & Cacheline (64B)  & High \\
    %    FPM & Low & One subarray & Row (8KB) & Low\\
    %    PSM & Med. $\leftrightarrow$ High & All banks & Cacheline (64B) &
    %    Med.\\
    %    \lisarc & Low $\leftrightarrow$ Med. & One bank & Cacheline
    %    $\leftrightarrow$  Row & Low\\

    %    \bottomrule
    %\end{tabular}
    \caption{Comparison of copy mechanism properties.}
  \label{tab:copy_tradeoff}%
\end{footnotesize}
\end{table}


==> sec/tables/dram_cmds.tex <==
\begin{table}[h]
\begin{footnotesize}
  \centering
    %\setlength{\tabcolsep}{.55em}
    \begin{tabular}{llr}
        \toprule
        Commands & Timing Parameters & Time (ns) \\
        \cmidrule(rl){1-3}
        \act $\rightarrow$ \crd/\cwr & \trcd & 13.75ns \\
        \crd $\rightarrow$ Data & \tcl & 13.75ns \\
        \cwr $\rightarrow$ Data & \tcwl & 10ns \\
        \act $\rightarrow$ \cpre & \tras & 35ns \\
        \cpre $\rightarrow$ \act & \trp & 13.75ns \\
        \bottomrule
    \end{tabular}
    \caption{Timing parameters for DRAM commands in DDR3-1600~\cite{jedec-ddr3}.}
  \label{tab:timing_parameters}%
\end{footnotesize}
\end{table}


==> sec/tables/intro_opt.tex <==
\begin{table}[h]
\begin{small}
  \centering
    \setlength{\tabcolsep}{.50em}
    \begin{tabular}{ll}
        \toprule
        %Index & Description\\
        %\cmidrule(rl){1-4}
        1. & A new bulk-data copy mechanism that uses \lisa to transfer data. \\
        \cmidrule(rl){1-2}

        2. & Precharge subarrays with two precharge units. \\
        \cmidrule(rl){1-2}

        \multirow{2}{*}{3.} & Use \lisa to perform fast in-DRAM caching in \\
                            & a heterogeneous DRAM with fast and slow subarrays. \\
        \cmidrule(rl){1-2}

        \multirow{2}{*}{4.} & Reduce subarray conflicts among frequently \\
                            & accessed rows when subarray-level parallelism is employed. \\

        \cmidrule(rl){1-2}

        \multirow{2}{*}{4.} & Enable fast collocation of frequently accessed \\
                            & sub-pages into a small number of row. \\
        \bottomrule
    \end{tabular}
    \caption{A list of optimizations enabled by \lisa.}
  \label{tab:intro_opt}
\end{small}
\end{table}


==> sec/tables/intro_opt_wide.tex <==
\begin{table*}[b]
    \begin{small}
        \centering
        %\setlength{\tabcolsep}{.40em}
        \begin{tabular}{p{1.5in}p{3.50in}p{1.78in}}
            \toprule
            \textbf{Problem} & \textbf{Mechanism LISA Enables}  & \textbf{Key
        System Benefits} \\
            \cmidrule(rl){1-3}
            \multirow{3}{*}{\minipage{1.5in}Slow inter-subarray data copying (1363.75ns for
            8KB). \refsec{lisaclone}\endminipage}&
                \underline{\lisarc}$\dagger$: Use \lisa to
            copy data between subarrays in the same bank with short latency --
            151ns, 88.9\% latency and 97.9\% DRAM energy
            reduction over prior work~\cite{seshadri-micro2013}.
            & 59.6\% system performance gain and 53.6\% DRAM energy reduction on
            a 4-core system.\\

            \cmidrule(rl){1-3}
            %High migration cost between heterogeneous subarrays. \refsec{villa}
            High memory access latency. \refsec{villa}
            & \underline{\lisavilla}$\dagger$: We add fast subarrays for caching
            in every bank and use \lisa to migrate/cache data.
            & Up to 16.1\% performance improvement and 5.1\% on average.\\

            \cmidrule(rl){1-3}
            \multirow{3}{*}{\minipage{1.5in}Slow precharge time (13.75ns).
            \refsec{lisapre}\endminipage} &
            \underline{\lisapre}$\dagger$: Use an extra
            precharge unit from the neighbor's subarray through \lisa to accelerate
            the precharge process (5ns -- 63.6\% latency reduction). &
            Up to 13.2\% performance improvement and 8.1\% on average.\\
            %8.1\% system performance gain and X\% DRAM energy reduction on
            %a 4-core system.\\

            %in a heterogeneous DRAM that adds fast subarrays for caching in every
            %bank. & 3.2\% average and 7.9\% maximum performance improvement.\\
            %Slow data transfers inhibit a DRAM design that adds
            %small, fast subarrays as caches. \refsec{villa}
            %& \underline{\lisavilla}$\dagger$: Use \lisa to transfer/cache data in a
            %heterogeneous DRAM that adds fast subarrays for caching in every
            %bank. & 3.2\% average and 7.9\% maximum performance improvement.\\

            \cmidrule(rl){1-3}
            \multirow{2}{*}{Subarray conflicts. \refsec{sa_remap}} & Remaps conflict-inflicting
            rows to different subarrays through \lisa when subarray-level
            parallelism~\cite{kim-isca2012} is employed. & Latency reduction due
            to fewer subarray conflicts. \\

            \cmidrule(rl){1-3} High-cost implementation of
            micro-pages~\cite{sudan-asplos2010}. \refsec{micro_pages} & \lisa enables an efficient
            implementation of prior work that collocates frequently accessed
            sub-pages into a small number of rows. & Performance improvement of
            micro-pages at low cost.\\

            \bottomrule
            \multicolumn{3}{r}{$\dagger$: We quantitatively evaluate the first three optimizations
            in this work.}
        \end{tabular}
        \caption{A list of optimizations \lisa enables.}
        \label{tab:intro_opt_wide}
    \end{small}
\end{table*}

%Slow data transfer latency from slow subarrays to fast subarrays for caching


==> sec/tables/migration_opt.tex <==
\begin{table*}[b]
    \begin{small}
        \centering
        %\setlength{\tabcolsep}{.40em}
        \begin{tabular}{p{1.45in}p{2.96in}p{2.1in}}

            \toprule
            \textbf{Problem} & \textbf{Mechanism LISA Enables}  & \textbf{Key
        System Benefits} \\
            \cmidrule(rl){1-3}
            \multirow{2}{*}{\minipage{1.5in}Slow inter-subarray data copying
            (\refsec{lisaclone})\endminipage} &
                \underline{\lisarcnol}$\dagger$:
                Bulk data copying between
                subarrays by exploiting LISA's \xfer operation.
                & Reduces (1) latency by 9.03x, (2)
                DRAM energy by 48.1x, over \rc~\cite{seshadri-micro2013}. \\
            %    --
            %151ns, 88.9\% latency reduction over prior work~\cite{seshadri-micro2013}.
            %& 59.6\% system performance gain and 53.6\% DRAM energy reduction.\\

            \cmidrule(rl){1-3}
            %High migration cost between heterogeneous subarrays. \refsec{villa}
            %Imbalanced heterogeneous DRAM designs~\cite{lee-hpca2013,son-isca2013}.

            High memory access latency (\refsec{villa}) &
            \underline{\lisavillanol}$\dagger$:
            Caches hot data via fast inter-subarray movement between
            heterogeneous subarrays within a bank.
            %Uses fast inter-subarray movement
            %to enable heterogeneous subarrays within a bank for caching.
            & Up to 16.1\% performance improvement (5.1\% on average) across 50 workloads.\\

            \cmidrule(rl){1-3}
            \multirow{2}{*}{\minipage{1.5in}Slow precharge time
            (\refsec{lisapre})\endminipage} &
            \underline{\lisaprenol}$\dagger$: Use extra
            precharge units from a neighboring subarray to accelerate the precharge
            process. & Up to 13.2\% performance improvement (8.1\% on average)
            across 50 workloads.\\

            \cmidrule(rl){1-3}
            \multirow{2}{*}{Subarray access conflicts} & Remaps conflicting rows in the
            same subarray to different subarrays when subarray-level
            parallelism~\cite{kim-isca2012} is employed. & Memory latency reduction due
            to fewer subarray conflicts. \\


            \cmidrule(rl){1-3} Costly row movement for \mbox{in-DRAM} Boolean
            logic~\cite{seshadri-cal2015} & Enables fast bulk bitwise AND and OR
            operations on two rows from \emph{different} subarrays. &
            Performance improvement from the extended range of bulk operations.
            \\

            %\cmidrule(rl){1-3} High-cost implementation of
            %micro-pages~\cite{sudan-asplos2010}. & Enable an efficient
            %implementation to quickly colocate frequently accessed
            %sub-pages into a small number of rows. & Performance improvement of
            %micro-pages at low cost.\\

            \bottomrule
            \multicolumn{3}{r}{$\dagger$: We quantitatively evaluate these optimizations in this work.}
        \end{tabular}
        \caption{A list of optimizations that benefit from \lisa's fast inter-subarray
        data movement.}
        \label{tab:migration_opt}
    \end{small}
\end{table*}

%Slow data transfer latency from slow subarrays to fast subarrays for caching


==> sec/tables/migration_opt_short.tex <==
\begin{table*}[b]
    \begin{small}
        \centering
        %\setlength{\tabcolsep}{.40em}
        \renewcommand{\arraystretch}{0.8}
        \begin{tabular}{p{1.45in}p{2.96in}p{2.1in}}

            \toprule
            \textbf{Problem} & \textbf{Mechanism LISA Enables}  & \textbf{Key
        System Benefits} \\

            \cmidrule(rl){1-3}
            \multirow{2}{*}{Subarray access conflicts} & Remaps conflicting rows in the
            same subarray to different subarrays when subarray-level
            parallelism~\cite{kim-isca2012} is employed. & Memory latency reduction due
            to fewer subarray conflicts. \\


            \cmidrule(rl){1-3} Costly row movement for \mbox{in-DRAM} Boolean
            logic~\cite{seshadri-cal2015} & Enables fast bulk bitwise AND and OR
            operations on two rows from \emph{different} subarrays. &
            Performance improvement from the extended range of bulk logic operations.
            \\

            %\cmidrule(rl){1-3} High-cost implementation of
            %micro-pages~\cite{sudan-asplos2010}. & Enable an efficient
            %implementation to quickly colocate frequently accessed
            %sub-pages into a small number of rows. & Performance improvement of
            %micro-pages at low cost.\\

            \bottomrule
        \end{tabular}
        \caption{Some additional applications that benefit from \lisa's fast inter-subarray
        data movement.}
        \label{tab:migration_opt_short}
    \end{small}
\end{table*}

%Slow data transfer latency from slow subarrays to fast subarrays for caching


==> sec/tables/sys_config_table.tex <==
%%%%%%%%%%%%%%%%%
% Single Column
%%%%%%%%%%%%%%%%%
\begin{table}[h]
    % \footnotesize
    %\small
    \fontsize{8.5}{10.2}\selectfont
    \renewcommand{\arraystretch}{0.8}
    \newdimen\origwspace
    \origwspace=\fontdimen2\font% original inter-word space
    %\fontdimen2\font=0.22em% decrease inter word space

    \centering
    \setlength{\tabcolsep}{.3em}
    \begin{tabular}{ll}
        \toprule
        \textbf{Processor} & 1--4 OoO cores, 4GHz, 3-wide issue \\
        \midrule

        \textbf{Cache} & L1: 64KB, L2: 512KB per core, L3: 4MB, 64B lines \\
        \midrule

        \textbf{Mem. Controller} & 64/64-entry read/write queue,
        FR-FCFS~\cite{rixner-isca2000,zuravleff-patent} \\

        %Memory & \multirow{2}{*}{64/64-entry read/write request queue,
        %FR-FCFS~\cite{rixner-isca2000}} \\
        %Controller & \\
        \midrule

        \multirow{2}{*}{\textbf{DRAM}} & DDR3-1600~\cite{micronDDR3_4Gb}, 1--2 channels, 1
        rank/channel,\\
        & 8 banks/rank, 16 subarrays/bank \\

        %\multirow{2}{*}{DRAM IDD (mA)} & IDD0=75, IDD2P=37, IDD2N=50, IDD3N=57, \\
        %                               & IDD4R=187, IDD4W=155 \\
        \bottomrule
    \end{tabular}
    \fontdimen2\font=\origwspace
    \caption{Evaluated system configuration.}
    \label{tab:sys-config}%
\end{table}


==> sec/tables/wkld_mixes.tex <==
%\begin{table}[h]
%\begin{footnotesize}
%  \centering
%    %\setlength{\tabcolsep}{.3em}
%    \begin{tabular}{ll}
%        \toprule
%        \multicolumn{2}{c}{\textbf{Copy Workloads}} \\
%        \midrule
%        CW 1 & tpcc64, forkbench, libquantum, bootup \\
%        CW 2 & bootup, xalancbmk, pagerank, forkbench \\
%        CW 3 & libquantum, pagerank, forkbench, bootup \\
%        CW 4 & mcf, forkbench, random, forkbench \\
%        CW 5 & bfs, bootup, tpch2, bootup \\
%        \midrule
%        \midrule
%        \multicolumn{2}{c}{\textbf{Memory-Intensive Workloads}} \\
%        \midrule
%        MW 1 & tpcc64, forkbench, libquantum, bootup \\
%        MW 2 & bootup, xalancbmk, pagerank, forkbench \\
%        MW 3 & libquantum, pagerank, forkbench, bootup \\
%        MW 4 & mcf, forkbench, random, forkbench \\
%        MW 5 & bfs, bootup, tpch2, bootup \\
%        \bottomrule
%    \end{tabular}
%  \caption{A subset of workload mixes that will be presented with detailed
%  results.}
%  \label{tab:wkld-mixes}%
%\end{footnotesize}
%\end{table}

\begin{table}[h]
    \small
    \centering
    %\setlength{\tabcolsep}{.3em}
    \renewcommand{\arraystretch}{0.8}
    \begin{tabular}{ll}
        \toprule
        %\multicolumn{2}{c}{\textbf{Copy Workloads}} \\
        %\midrule
        \textbf{Mix 1} & \texttt{tpcc64, forkbench, libquantum, bootup} \\
        \textbf{Mix 2} & \texttt{bootup, xalancbmk, pagerank, forkbench} \\
        \textbf{Mix 3} & \texttt{libquantum, pagerank, forkbench, bootup} \\
        \textbf{Mix 4} & \texttt{mcf, forkbench, random, forkbench} \\
        \textbf{Mix 5} & \texttt{bfs, bootup, tpch2, bootup} \\
        \bottomrule
    \end{tabular}
    \caption{A subset of copy workloads with detailed results.}
    \label{tab:wkld-mixes}%
\end{table}

